Fusing Gathers with Integer Linear Programming

We present an Integer Linear Programming based approach to finding the optimal fusion strategy for combinator-based parallel programs. While combinator-based languages or libraries provide a convenient interface for programming parallel hardware, fusing combinators to more complex operations is essential to achieve the desired performance. Our approach is not only suitable for languages with the usual map, fold, scan, indexing and scatter operations, but also gather operations, which access arrays in arbitrary order, and therefore goes beyond the traditional producer-consumer fusion. It can be parametrised with appropriate cost functions, and is fast enough to be suitable for just-in-time compilation.

==> benchmarks/complexgraph.tex <==
\begin{figure}[t]


  % it's slightly wide now perhaps; when this was still 3 tikz pictures they were not vertically aligned but the space between them was slightly smaller. See commit 7cdc0225339a59f1959b28312478fb9e1fac4e2c
  \begin{tikzpicture}
      \node (xs1)                               {xs};
      \node (as1) [below of=xs1, left of=xs1  ] {as};
      \node (bs1) [below of=xs1, right of=xs1 ] {bs};
      \node (cs1) [below of=as1               ] {cs};
      \node (ds1) [below of=bs1               ] {ds};
      \draw[-{Implies},double] (xs1) -- (as1);
      \draw[-{Implies},double] (xs1) -- (bs1);
      \draw[->]                (as1) -- (cs1);
      \draw[->]                (bs1) -- (ds1);
      \draw[-{Implies},double] (as1) -- (ds1);
      \draw[-{Implies},double] (bs1) -- (cs1);
      \draw (0,-1) circle [x radius=1.3, y radius =0.3];
      \draw (0,-2) circle [x radius=1.3, y radius =0.3];
      
      \node (as2) [right of=bs1               ] {as};
      \node (xs2) [above of=as2, right of=as2 ] {xs};
      \node (bs2) [below of=xs2, right of=xs2 ] {bs};
      \node (cs2) [below of=as2               ] {cs};
      \node (ds2) [below of=bs2               ] {ds};
      \draw[-{Implies},double] (xs2) -- (as2);
      \draw[-{Implies},double] (xs2) -- (bs2);
      \draw[->]                (as2) -- (cs2);
      \draw[->]                (bs2) -- (ds2);
      \draw[-{Implies},double] (as2) -- (ds2);
      \draw[-{Implies},double] (bs2) -- (cs2);
      \draw (2,-1.5) circle [x radius=.4, y radius =1];
      \draw (4,-1) circle [radius = .4];
      \draw (4,-2) circle [radius = .4];
      
      \node (as3) [right of=bs2               ] {as};
      \node (xs3) [above of=as3, right of=as3 ] {xs};
      \node (bs3) [below of=xs3, right of=xs3 ] {bs};
      \node (cs3) [below of=as3               ] {cs};
      \node (ds3) [below of=bs3               ] {ds};
      \draw[-{Implies},double] (xs3) -- (as3);
      \draw[-{Implies},double] (xs3) -- (bs3);
      \draw[->]                (as3) -- (cs3);
      \draw[->]                (bs3) -- (ds3);
      \draw[-{Implies},double] (as3) -- (ds3);
      \draw[-{Implies},double] (bs3) -- (cs3);
      \draw (7,-1.5) circle [x radius=.4, y radius =1];
      \draw (5,-1) circle [radius = .4];
      \draw (5,-2) circle [radius = .4];
  \end{tikzpicture}
  \caption{Possible clusterings of the function \lstinline{complex}}\label{fig:complexgraph}
\end{figure}

==> benchmarks/difficultgraph.tex <==
\begin{figure}[t]
  \begin{tikzpicture}
    \node (ys1)                               {ys};
    \node (xs1) [above of=ys1]                {xs};
    \node (as1) [below of=ys1, left of=ys1  ] {as};
    \node (bs1) [below of=ys1, right of=ys1 ] {bs};
    \node (cs1) [below of=as1               ] {cs};
    \node (ds1) [below of=bs1               ] {ds};
    \draw[->]                (xs1) -- (ys1);
    \draw[->]                (ys1) -- (as1);
    \draw[->]                (ys1) -- (bs1);
    \draw[->]                (as1) -- (cs1);
    \draw[->]                (bs1) -- (ds1);
    \draw[-{Implies},double] (as1) -- (ds1);
    \draw[-{Implies},double] (bs1) -- (cs1);
    % \begin{scope}[rotate around={45:(-0.5,-0.5)}]
    %   \draw[dotted] (-0.5,-0.5) circle [x radius=1.2, y radius=0.3];
    % \end{scope}
    % \draw[dotted] ( 1  ,-1.5) circle [x radius=0.3, y radius=1  ];
    % \draw[dotted] (-1  ,-2  ) circle [x radius=0.3, y radius=0.3];
    \draw ( 0,-0.7 ) circle [x radius=1.3, y radius=0.9];
    \draw (-1,-2   ) circle [x radius=0.3, y radius=0.3];
    \draw ( 1,-2   ) circle [x radius=0.3, y radius=0.3];
  \end{tikzpicture}
  \begin{tikzpicture}
    \node (ys1)                               {ys};
    \node (xs1) [above of=ys1]                {xs};
    \node (as1) [below of=ys1, left of=ys1  ] {as};
    \node (bs1) [below of=ys1, right of=ys1 ] {bs};
    \node (cs1) [below of=as1               ] {cs};
    \node (ds1) [below of=bs1               ] {ds};
    \draw[->]                (xs1) -- (ys1);
    \draw[->]                (ys1) -- (as1);
    \draw[->]                (ys1) -- (bs1);
    \draw[->]                (as1) -- (cs1);
    \draw[->]                (bs1) -- (ds1);
    \draw[-{Implies},double] (as1) -- (ds1);
    \draw[-{Implies},double] (bs1) -- (cs1);
    \begin{scope}[rotate around={45:(-0.5,-0.5)}]
      \draw (-0.5,-0.5) circle [x radius=1.2, y radius=0.3];
    \end{scope}
    \draw (-1,-2   ) circle [x radius=0.3, y radius=0.3];
    \draw ( 1,-1.5 ) circle [x radius=0.3, y radius=0.8];
    % \draw[dashed] (-1.3, 0.3) rectangle ++( 2.6,-1.7);
    % \draw[dashed] ( 0.7,-2.3) rectangle ++( 0.6, 0.6);
    % \draw[dashed] (-0.7,-2.3) rectangle ++(-0.6, 0.6);
  \end{tikzpicture}
  \caption{Optimal (left) and Futhark (right) clusterings of the function \lstinline{mapComplex}}\label{fig:difficultgraph}
\end{figure}

==> clustering/diagonal.tex <==
\subsection{Fusing Clusters}\label{sec:diagonal}

Let us start our discussion on the effects of fusion with the two most common fusion methods, often called \emph{vertical fusion} and \emph{horizontal fusion}
in the existing literature~\cite{streamprocessing}.
%
Informally, \emph{vertical fusion} pipes the result of one cluster as input into another, eliminating the need to store the intermediate
result, as shown in Figure~\ref{fig:vertical}.
%
\emph{Horizontal fusion}, on the other hand, describes the fusion of two clusters which consume the same input, as in Figure~\ref{fig:horizontal}. The fused cluster here produces as output both of the outputs of the two individual clusters. Horizontal fusion reduces memory traffic, as it's only necessary to
access the elements of the input array once to produce both outputs.

% We can identify two more methods of fusion.
% Firstly, \emph{independent fusion}: two clusters which might not have any data dependencies, but still share the same iteration size.
% % For example, @cs@ and @ds@ in the first clustering in Figure \ref{fig:clusterings} are independent.
% This means that they are fusible, but we do not eliminate any memory accesses by fusing these loops. While for
% horizontal and vertical fusion the benefits are usually clear, the situation is more subtle here: it can be advantageous
% that the loops can share their counters and control flow, but there are also cases
% where this class of fusion has no positive effect.

There is another interesting case which we shall call \emph{diagonal fusion},
as shown in Figure~\ref{fig:diagonal}.
It is similar to vertical fusion, in that one cluster consumes the result of the
other, but this intermediate result is retained.
% The second clustering in Figure \ref{fig:clusterings} showcases an application of diagonal fusion: The intermediate array @as@ cannot be eliminated using vertical fusion, because it is still required in order to compute @ds@.
Diagonally fusing two loops has only some of the performance benefits of vertically fusing them, as the memory read from the second loop is eliminated but the write from the first loop is still required, but it is less restrictive and is thus more often applicable.
% Figure \ref{fig:verhordiag} graphically displays the three non-independent variants on a data dependence graph.

% It is possible to express diagonal fusion using vertical fusion, horizontal fusion and @map id@, but ....

% \tlm{at this point I think it would be enlightening to point out how diagonal
% fusion relates to the usual horizontal and vertical cases. possible thought
% process of the reader: ``isn't diagonal just horizontal fusion where one of the
% functions is \texttt{map id}? oh but I guess you did something to the input
% first, but that's just vertical fusion? so isn't that already covered by the
% combination of these two things (i.e. existing work) and why do we need to name
% it explicitly?'' I feel like that's an interesting point to make here and I
% missed it.}
% \dvb{I don't mind saying this, see the last sentence above, but I find it hard to articulate why we do want
% explicit diagonal fusion (so we don't need to introduce extra 'map id's is a big one, because I don't want 
% the construction in 3.3 to have to add new combinators, but it also just simplifies the exposition as well as the implementation).}
% \gck{need to write more once I understand properly why its useful}

